A Pilot Study of Nulling in 22 Pulsars Using Mixture Modeling

The phenomenon of pulsar nulling, observed as the temporary inactivity of a pulsar, remains poorly understood both observationally and theoretically. Most observational studies that quantify nulling employ a variant of Ritchings (1976)'s algorithm which can suffer significant biases for pulsars where the emission is weak. Using a more robust mixture model method, we study pulsar nulling in a sample of 22 recently discovered pulsars, for which we publish the nulling fractions for the first time. These data clearly demonstrate biases of the former approach and show how an otherwise non-nulling pulsar can be classified as having significant nulls. We show that the population-wide studies that find a positive correlation of nulling with pulsar period/characteristic age can similarly be biased because of the bias in estimating the nulling fraction. We use our probabilistic approach to find the evidence for periodicity in the nulls in a subset of three pulsars in our sample. In addition, we also provide improved timing parameters for 17 of the 22 pulsars that had no prior follow-up.

==> all_figures_online.tex <==
\figsetstart
\figsetnum{3}
\figsettitle{Single pulse stacks and mixture model fits for all the pulsars}

\figsetgrpstart
\figsetgrpnum{3.1}
\figsetgrptitle{PSR J0054+6946}
\figsetplot{figures/all_pulsars/J0054+6946/dspsr_fold/J0054+6946_profile_sps_paper_version.pdf}
\figsetplot{figures/all_pulsars/J0054+6946/dspsr_fold/J0054+6946_corner_plot_paper_version.pdf}
\centerline{\figsetplot{figures/all_pulsars/J0054+6946/dspsr_fold/J0054+6946_hist_fit_paper_version.pdf}}
\figsetgrpnote{Single pulse stack (upper left), MCMC corner plot (bottom), and pulse intensity histogram (upper right) with the best fit model, a 2-component Gaussian mixture}
\figsetgrpend


\figsetgrpstart
\figsetgrpnum{3.2}
\figsetgrptitle{PSR J0111+6624}
\figsetplot{figures/all_pulsars/J0111+6624/dspsr_fold/J0111+6624_profile_sps_paper_version.pdf}
\figsetplot{figures/all_pulsars/J0111+6624/dspsr_fold/J0111+6624_corner_plot_paper_version.pdf}
\centerline{\figsetplot{figures/all_pulsars/J0111+6624/dspsr_fold/J0111+6624_hist_fit_paper_version.pdf}}
\figsetgrpnote{Single pulse stack (upper left), MCMC corner plot (bottom), and pulse intensity histogram (upper right) with the best fit model, a 2-component Gaussian mixture}
\figsetgrpend


\figsetgrpstart
\figsetgrpnum{3.3}
\figsetgrptitle{PSR J0325+6744}
\figsetplot{figures/all_pulsars/J0325+6744/dspsr_fold/J0325+6744_profile_sps_paper_version.pdf}
\figsetplot{figures/all_pulsars/J0325+6744/dspsr_fold/J0325+6744_corner_plot_paper_version.pdf}
\centerline{\figsetplot{figures/all_pulsars/J0325+6744/dspsr_fold/J0325+6744_hist_fit_paper_version.pdf}}
\figsetgrpnote{Single pulse stack (upper left), MCMC corner plot (bottom), and pulse intensity histogram (upper right) with the best fit model, a 2-component Gaussian mixture}
\figsetgrpend


\figsetgrpstart
\figsetgrpnum{3.4}
\figsetgrptitle{PSR J0355+28}
\figsetplot{figures/all_pulsars/J0355+28/dspsr_fold/J0355+28_profile_sps_paper_version.pdf}
\figsetplot{figures/all_pulsars/J0355+28/dspsr_fold/J0355+28_corner_plot_paper_version.pdf}
\centerline{\figsetplot{figures/all_pulsars/J0355+28/dspsr_fold/J0355+28_hist_fit_paper_version.pdf}}
\figsetgrpnote{Single pulse stack (upper left), MCMC corner plot (bottom), and pulse intensity histogram (upper right) with the best fit model, a 2-component Gaussian mixture}
\figsetgrpend


\figsetgrpstart
\figsetgrpnum{3.5}
\figsetgrptitle{PSR J0414+31 (GBT)}
\figsetplot{figures/all_pulsars/J0414+31_GBT/dspsr_fold/J0414+31_GBT_profile_sps_paper_version.pdf}
\figsetplot{figures/all_pulsars/J0414+31_GBT/dspsr_fold/J0414+31_GBT_corner_plot_paper_version.pdf}
\centerline{\figsetplot{figures/all_pulsars/J0414+31_GBT/dspsr_fold/J0414+31_GBT_hist_fit_paper_version.pdf}}
\figsetgrpnote{Single pulse stack (upper left), MCMC corner plot (bottom), and pulse intensity histogram (upper right) with the best fit model, a 2-component Gaussian mixture}
\figsetgrpend


\figsetgrpstart
\figsetgrpnum{3.6}
\figsetgrptitle{PSR J0414+31 (AO)}
\figsetplot{figures/all_pulsars/J0414+31_arecibo/dspsr_fold/J0414+31_arecibo_profile_sps_paper_version.pdf}
\figsetplot{figures/all_pulsars/J0414+31_arecibo/dspsr_fold/J0414+31_arecibo_corner_plot_paper_version.pdf}
\centerline{\figsetplot{figures/all_pulsars/J0414+31_arecibo/dspsr_fold/J0414+31_arecibo_hist_fit_paper_version.pdf}}
\figsetgrpnote{Single pulse stack (upper left), MCMC corner plot (bottom), and pulse intensity histogram (upper right) with the best fit model, a 2-component Gaussian mixture}
\figsetgrpend


\figsetgrpstart
\figsetgrpnum{3.7}
\figsetgrptitle{PSR J0614+83}
\figsetplot{figures/all_pulsars/J0614+83/dspsr_fold/J0614+83_profile_sps_paper_version.pdf}
\figsetplot{figures/all_pulsars/J0614+83/dspsr_fold/J0614+83_corner_plot_paper_version.pdf}
\centerline{\figsetplot{figures/all_pulsars/J0614+83/dspsr_fold/J0614+83_hist_fit_paper_version.pdf}}
\figsetgrpnote{Single pulse stack (upper left), MCMC corner plot (bottom), and pulse intensity histogram (upper right) with the best fit model, a 2-component Gaussian mixture}
\figsetgrpend


\figsetgrpstart
\figsetgrpnum{3.8}
\figsetgrptitle{PSR J0738+6904}
\figsetplot{figures/all_pulsars/J0738+6904/dspsr_fold/J0738+6904_profile_sps_paper_version.pdf}
\figsetplot{figures/all_pulsars/J0738+6904/dspsr_fold/J0738+6904_corner_plot_paper_version.pdf}
\centerline{\figsetplot{figures/all_pulsars/J0738+6904/dspsr_fold/J0738+6904_hist_fit_paper_version.pdf}}
\figsetgrpnote{Single pulse stack (upper left), MCMC corner plot (bottom), and pulse intensity histogram (upper right) with the best fit model, a 2-component Gaussian mixture}
\figsetgrpend


\figsetgrpstart
\figsetgrpnum{3.9}
\figsetgrptitle{PSR J1529-26}
\figsetplot{figures/all_pulsars/J1529-26/dspsr_fold/J1529-26_profile_sps_paper_version.pdf}
\figsetplot{figures/all_pulsars/J1529-26/dspsr_fold/J1529-26_corner_plot_paper_version.pdf}
\centerline{\figsetplot{figures/all_pulsars/J1529-26/dspsr_fold/J1529-26_hist_fit_paper_version.pdf}}
\figsetgrpnote{Single pulse stack (upper left), MCMC corner plot (bottom), and pulse intensity histogram (upper right) with the best fit model, a 2-component Gaussian mixture}
\figsetgrpend


\figsetgrpstart
\figsetgrpnum{3.10}
\figsetgrptitle{PSR J1536-30}
\figsetplot{figures/all_pulsars/J1536-30/dspsr_fold/J1536-30_profile_sps_paper_version.pdf}
\figsetplot{figures/all_pulsars/J1536-30/dspsr_fold/J1536-30_corner_plot_paper_version.pdf}
\centerline{\figsetplot{figures/all_pulsars/J1536-30/dspsr_fold/J1536-30_hist_fit_paper_version.pdf}}
\figsetgrpnote{Single pulse stack (upper left), MCMC corner plot (bottom), and pulse intensity histogram (upper right) with the best fit model, a 2-component Gaussian mixture}
\figsetgrpend


\figsetgrpstart
\figsetgrpnum{3.11}
\figsetgrptitle{PSR J1629+33}
\figsetplot{figures/all_pulsars/J1629+33/dspsr_fold/J1629+33_profile_sps_paper_version.pdf}
\figsetplot{figures/all_pulsars/J1629+33/dspsr_fold/J1629+33_corner_plot_paper_version.pdf}
\centerline{\figsetplot{figures/all_pulsars/J1629+33/dspsr_fold/J1629+33_hist_fit_paper_version.pdf}}
\figsetgrpnote{Single pulse stack (upper left), MCMC corner plot (bottom), and pulse intensity histogram (upper right) with the best fit model, a 2-component Gaussian mixture}
\figsetgrpend


\figsetgrpstart
\figsetgrpnum{3.12}
\figsetgrptitle{PSR J1821+4147}
\figsetplot{figures/all_pulsars/J1821+4147/dspsr_fold/J1821+4147_profile_sps_paper_version.pdf}
\figsetplot{figures/all_pulsars/J1821+4147/dspsr_fold/J1821+4147_corner_plot_paper_version.pdf}
\centerline{\figsetplot{figures/all_pulsars/J1821+4147/dspsr_fold/J1821+4147_hist_fit_paper_version.pdf}}
\figsetgrpnote{Single pulse stack (upper left), MCMC corner plot (bottom), and pulse intensity histogram (upper right) with the best fit model, a 2-component Gaussian mixture}
\figsetgrpend


\figsetgrpstart
\figsetgrpnum{3.13}
\figsetgrptitle{PSR J1822+02}
\figsetplot{figures/all_pulsars/J1822+02/dspsr_fold/J1822+02_profile_sps_paper_version.pdf}
\figsetplot{figures/all_pulsars/J1822+02/dspsr_fold/J1822+02_corner_plot_paper_version.pdf}
\centerline{\figsetplot{figures/all_pulsars/J1822+02/dspsr_fold/J1822+02_hist_fit_paper_version.pdf}}
\figsetgrpnote{Single pulse stack (upper left), MCMC corner plot (bottom), and pulse intensity histogram (upper right) with the best fit model, a 2-component Gaussian mixture}
\figsetgrpend


\figsetgrpstart
\figsetgrpnum{3.14}
\figsetgrptitle{PSR J1829+25}
\figsetplot{figures/all_pulsars/J1829+25/dspsr_fold/J1829+25_profile_sps_paper_version.pdf}
\figsetplot{figures/all_pulsars/J1829+25/dspsr_fold/J1829+25_corner_plot_paper_version.pdf}
\centerline{\figsetplot{figures/all_pulsars/J1829+25/dspsr_fold/J1829+25_hist_fit_paper_version.pdf}}
\figsetgrpnote{Single pulse stack (upper left), MCMC corner plot (bottom), and pulse intensity histogram (upper right) with the best fit model, a 2-component Gaussian mixture}
\figsetgrpend


\figsetgrpstart
\figsetgrpnum{3.15}
\figsetgrptitle{PSR J1829+25}
\figsetplot{figures/all_pulsars/J1829+25_GBT/dspsr_fold/J1829+25_profile_sps_paper_version.pdf}
\figsetplot{figures/all_pulsars/J1829+25_GBT/dspsr_fold/J1829+25_corner_plot_paper_version.pdf}
\centerline{\figsetplot{figures/all_pulsars/J1829+25_GBT/dspsr_fold/J1829+25_hist_fit_paper_version.pdf}}
\figsetgrpnote{Single pulse stack (upper left), MCMC corner plot (bottom), and pulse intensity histogram (upper right) with the best fit model, a 2-component Gaussian mixture}
\figsetgrpend


\figsetgrpstart
\figsetgrpnum{3.16}
\figsetgrptitle{PSR J1901-04}
\figsetplot{figures/all_pulsars/J1901-04/dspsr_fold/J1901-04_profile_sps_paper_version.pdf}
\figsetplot{figures/all_pulsars/J1901-04/dspsr_fold/J1901-04_corner_plot_paper_version.pdf}
\centerline{\figsetplot{figures/all_pulsars/J1901-04/dspsr_fold/J1901-04_hist_fit_paper_version.pdf}}
\figsetgrpnote{Single pulse stack (upper left), MCMC corner plot (bottom), and pulse intensity histogram (upper right) with the best fit model, a 2-component Gaussian mixture}
\figsetgrpend


\figsetgrpstart
\figsetgrpnum{3.17}
\figsetgrptitle{PSR J1904+33}
\figsetplot{figures/all_pulsars/J1904+33/dspsr_fold/J1904+33_profile_sps_paper_version.pdf}
\figsetplot{figures/all_pulsars/J1904+33/dspsr_fold/J1904+33_corner_plot_paper_version.pdf}
\centerline{\figsetplot{figures/all_pulsars/J1904+33/dspsr_fold/J1904+33_hist_fit_paper_version.pdf}}
\figsetgrpnote{Single pulse stack (upper left), MCMC corner plot (bottom), and pulse intensity histogram (upper right) with the best fit model, a 2-component Gaussian mixture}
\figsetgrpend


\figsetgrpstart
\figsetgrpnum{3.18}
\figsetgrptitle{PSR J1928+28}
\figsetplot{figures/all_pulsars/J1928+28/dspsr_fold/J1928+28_profile_sps_paper_version.pdf}
\figsetplot{figures/all_pulsars/J1928+28/dspsr_fold/J1928+28_corner_plot_paper_version.pdf}
\centerline{\figsetplot{figures/all_pulsars/J1928+28/dspsr_fold/J1928+28_hist_fit_paper_version.pdf}}
\figsetgrpnote{Single pulse stack (upper left), MCMC corner plot (bottom), and pulse intensity histogram (upper right) with the best fit model, a 2-component Gaussian mixture}
\figsetgrpend


\figsetgrpstart
\figsetgrpnum{3.19}
\figsetgrptitle{PSR J1941+02}
\figsetplot{figures/all_pulsars/J1941+02/dspsr_fold/J1941+02_profile_sps_paper_version.pdf}
\figsetplot{figures/all_pulsars/J1941+02/dspsr_fold/J1941+02_corner_plot_paper_version.pdf}
\centerline{\figsetplot{figures/all_pulsars/J1941+02/dspsr_fold/J1941+02_hist_fit_paper_version.pdf}}
\figsetgrpnote{Single pulse stack (upper left), MCMC corner plot (bottom), and pulse intensity histogram (upper right) with the best fit model, a 2-component Gaussian mixture}
\figsetgrpend


\figsetgrpstart
\figsetgrpnum{3.20}
\figsetgrptitle{PSR J2000+29}
\figsetplot{figures/all_pulsars/J2000+29/dspsr_fold/J2000+29_profile_sps_paper_version.pdf}
\figsetplot{figures/all_pulsars/J2000+29/dspsr_fold/J2000+29_corner_plot_paper_version.pdf}
\centerline{\figsetplot{figures/all_pulsars/J2000+29/dspsr_fold/J2000+29_hist_fit_paper_version.pdf}}
\figsetgrpnote{Single pulse stack (upper left), MCMC corner plot (bottom), and pulse intensity histogram (upper right) with the best fit model, a 2-component Gaussian mixture}
\figsetgrpend


\figsetgrpstart
\figsetgrpnum{3.21}
\figsetgrptitle{PSR J2040-21}
\figsetplot{figures/all_pulsars/J2040-21/dspsr_fold/J2040-21_profile_sps_paper_version.pdf}
\figsetplot{figures/all_pulsars/J2040-21/dspsr_fold/J2040-21_corner_plot_paper_version.pdf}
\centerline{\figsetplot{figures/all_pulsars/J2040-21/dspsr_fold/J2040-21_hist_fit_paper_version.pdf}}
\figsetgrpnote{Single pulse stack (upper left), MCMC corner plot (bottom), and pulse intensity histogram (upper right) with the best fit model, a 2-component Gaussian mixture}
\figsetgrpend


\figsetgrpstart
\figsetgrpnum{3.22}
\figsetgrptitle{PSR J2044+28}
\figsetplot{figures/all_pulsars/J2044+28/dspsr_fold/J2044+28_profile_sps_paper_version.pdf}
\figsetplot{figures/all_pulsars/J2044+28/dspsr_fold/J2044+28_corner_plot_paper_version.pdf}
\centerline{\figsetplot{figures/all_pulsars/J2044+28/dspsr_fold/J2044+28_hist_fit_paper_version.pdf}}
\figsetgrpnote{Single pulse stack (upper left), MCMC corner plot (bottom), and pulse intensity histogram (upper right) with the best fit model, a 2-component Gaussian mixture}
\figsetgrpend


\figsetgrpstart
\figsetgrpnum{3.23}
\figsetgrptitle{PSR J2131-31}
\figsetplot{figures/all_pulsars/J2131-31/dspsr_fold/J2131-31_profile_sps_paper_version.pdf}
\figsetplot{figures/all_pulsars/J2131-31/dspsr_fold/J2131-31_corner_plot_paper_version.pdf}
\centerline{\figsetplot{figures/all_pulsars/J2131-31/dspsr_fold/J2131-31_hist_fit_paper_version.pdf}}
\figsetgrpnote{Single pulse stack (upper left), MCMC corner plot (bottom), and pulse intensity histogram (upper right) with the best fit model, a 2-component Gaussian mixture}
\figsetgrpend


\figsetgrpstart
\figsetgrpnum{3.24}
\figsetgrptitle{PSR J2310+6706}
\figsetplot{figures/all_pulsars/J2310+6706/dspsr_fold/J2310+6706_profile_sps_paper_version.pdf}
\figsetplot{figures/all_pulsars/J2310+6706/dspsr_fold/J2310+6706_corner_plot_paper_version.pdf}
\centerline{\figsetplot{figures/all_pulsars/J2310+6706/dspsr_fold/J2310+6706_hist_fit_paper_version.pdf}}
\figsetgrpnote{Single pulse stack (upper left), MCMC corner plot (bottom), and pulse intensity histogram (upper right) with the best fit model, a 2-component Gaussian mixture}
\figsetgrpend

\figsetend
% \figsetgrpstart
% \figsetgrpnum{3.0}
% \figsetgrptitle{PSR J0054+6946}
% \figsetplot{figures/all_pulsars/J0054+6946/dspsr_fold/J0054+6946_profile_sps_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J0054+6946/dspsr_fold/J0054+6946_corner_plot_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J0054+6946/dspsr_fold/J0054+6946_hist_fit_paper_version.pdf}
% \figsetgrpnote{Pulse stack, Posteriors, ON/OFF histogram model fit}
% \figsetgrpend


% \figsetgrpstart
% \figsetgrpnum{3.1}
% \figsetgrptitle{PSR J0111+6624}
% \figsetplot{figures/all_pulsars/J0111+6624/dspsr_fold/J0111+6624_profile_sps_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J0111+6624/dspsr_fold/J0111+6624_corner_plot_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J0111+6624/dspsr_fold/J0111+6624_hist_fit_paper_version.pdf}
% \figsetgrpnote{Pulse stack, Posteriors, ON/OFF histogram model fit}
% \figsetgrpend


% \figsetgrpstart
% \figsetgrpnum{3.2}
% \figsetgrptitle{PSR J0325+6744}
% \figsetplot{figures/all_pulsars/J0325+6744/dspsr_fold/J0325+6744_profile_sps_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J0325+6744/dspsr_fold/J0325+6744_corner_plot_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J0325+6744/dspsr_fold/J0325+6744_hist_fit_paper_version.pdf}
% \figsetgrpnote{Pulse stack, Posteriors, ON/OFF histogram model fit}
% \figsetgrpend


% \figsetgrpstart
% \figsetgrpnum{3.3}
% \figsetgrptitle{PSR J0355+28}
% \figsetplot{figures/all_pulsars/J0355+28/dspsr_fold/J0355+28_profile_sps_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J0355+28/dspsr_fold/J0355+28_corner_plot_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J0355+28/dspsr_fold/J0355+28_hist_fit_paper_version.pdf}
% \figsetgrpnote{Pulse stack, Posteriors, ON/OFF histogram model fit}
% \figsetgrpend


% \figsetgrpstart
% \figsetgrpnum{3.4}
% \figsetgrptitle{PSR J0414+31 (GBT)}
% \figsetplot{figures/all_pulsars/J0414+31_GBT/dspsr_fold/J0414+31_GBT_profile_sps_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J0414+31_GBT/dspsr_fold/J0414+31_GBT_corner_plot_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J0414+31_GBT/dspsr_fold/J0414+31_GBT_hist_fit_paper_version.pdf}
% \figsetgrpnote{Pulse stack, Posteriors, ON/OFF histogram model fit}
% \figsetgrpend


% \figsetgrpstart
% \figsetgrpnum{3.5}
% \figsetgrptitle{PSR J0414+31 (AO)}
% \figsetplot{figures/all_pulsars/J0414+31_arecibo/dspsr_fold/J0414+31_arecibo_profile_sps_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J0414+31_arecibo/dspsr_fold/J0414+31_arecibo_corner_plot_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J0414+31_arecibo/dspsr_fold/J0414+31_arecibo_hist_fit_paper_version.pdf}
% \figsetgrpnote{Pulse stack, Posteriors, ON/OFF histogram model fit}
% \figsetgrpend


% \figsetgrpstart
% \figsetgrpnum{3.6}
% \figsetgrptitle{PSR J0614+83}
% \figsetplot{figures/all_pulsars/J0614+83/dspsr_fold/J0614+83_profile_sps_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J0614+83/dspsr_fold/J0614+83_corner_plot_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J0614+83/dspsr_fold/J0614+83_hist_fit_paper_version.pdf}
% \figsetgrpnote{Pulse stack, Posteriors, ON/OFF histogram model fit}
% \figsetgrpend


% \figsetgrpstart
% \figsetgrpnum{3.7}
% \figsetgrptitle{PSR J0738+6904}
% \figsetplot{figures/all_pulsars/J0738+6904/dspsr_fold/J0738+6904_profile_sps_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J0738+6904/dspsr_fold/J0738+6904_corner_plot_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J0738+6904/dspsr_fold/J0738+6904_hist_fit_paper_version.pdf}
% \figsetgrpnote{Pulse stack, Posteriors, ON/OFF histogram model fit}
% \figsetgrpend


% \figsetgrpstart
% \figsetgrpnum{3.8}
% \figsetgrptitle{PSR J1529$-$26}
% \figsetplot{figures/all_pulsars/J1529-26/dspsr_fold/J1529-26_profile_sps_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J1529-26/dspsr_fold/J1529-26_corner_plot_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J1529-26/dspsr_fold/J1529-26_hist_fit_paper_version.pdf}
% \figsetgrpnote{Pulse stack, Posteriors, ON/OFF histogram model fit}
% \figsetgrpend


% \figsetgrpstart
% \figsetgrpnum{3.9}
% \figsetgrptitle{PSR J1536$-$30}
% \figsetplot{figures/all_pulsars/J1536-30/dspsr_fold/J1536-30_profile_sps_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J1536-30/dspsr_fold/J1536-30_corner_plot_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J1536-30/dspsr_fold/J1536-30_hist_fit_paper_version.pdf}
% \figsetgrpnote{Pulse stack, Posteriors, ON/OFF histogram model fit}
% \figsetgrpend


% \figsetgrpstart
% \figsetgrpnum{3.10}
% \figsetgrptitle{PSR J1629+33}
% \figsetplot{figures/all_pulsars/J1629+33/dspsr_fold/J1629+33_profile_sps_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J1629+33/dspsr_fold/J1629+33_corner_plot_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J1629+33/dspsr_fold/J1629+33_hist_fit_paper_version.pdf}
% \figsetgrpnote{Pulse stack, Posteriors, ON/OFF histogram model fit}
% \figsetgrpend


% \figsetgrpstart
% \figsetgrpnum{3.11}
% \figsetgrptitle{PSR J1821+4147}
% \figsetplot{figures/all_pulsars/J1821+4147/dspsr_fold/J1821+4147_profile_sps_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J1821+4147/dspsr_fold/J1821+4147_corner_plot_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J1821+4147/dspsr_fold/J1821+4147_hist_fit_paper_version.pdf}
% \figsetgrpnote{Pulse stack, Posteriors, ON/OFF histogram model fit}
% \figsetgrpend


% \figsetgrpstart
% \figsetgrpnum{3.12}
% \figsetgrptitle{PSR J1822+02}
% \figsetplot{figures/all_pulsars/J1822+02/dspsr_fold/J1822+02_profile_sps_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J1822+02/dspsr_fold/J1822+02_corner_plot_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J1822+02/dspsr_fold/J1822+02_hist_fit_paper_version.pdf}
% \figsetgrpnote{Pulse stack, Posteriors, ON/OFF histogram model fit}
% \figsetgrpend


% \figsetgrpstart
% \figsetgrpnum{3.13}
% \figsetgrptitle{PSR J1829+25}
% \figsetplot{figures/all_pulsars/J1829+25/dspsr_fold/J1829+25_profile_sps_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J1829+25/dspsr_fold/J1829+25_corner_plot_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J1829+25/dspsr_fold/J1829+25_hist_fit_paper_version.pdf}
% \figsetgrpnote{Pulse stack, Posteriors, ON/OFF histogram model fit}
% \figsetgrpend


% \figsetgrpstart
% \figsetgrpnum{3.14}
% \figsetgrptitle{PSR J1829+25}
% \figsetplot{figures/all_pulsars/J1829+25/dspsr_fold/J1829+25_profile_sps_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J1829+25/dspsr_fold/J1829+25_corner_plot_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J1829+25/dspsr_fold/J1829+25_hist_fit_paper_version.pdf}
% \figsetgrpnote{Pulse stack, Posteriors, ON/OFF histogram model fit}
% \figsetgrpend


% \figsetgrpstart
% \figsetgrpnum{3.15}
% \figsetgrptitle{PSR J1901$-$04}
% \figsetplot{figures/all_pulsars/J1901-04/dspsr_fold/J1901-04_profile_sps_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J1901-04/dspsr_fold/J1901-04_corner_plot_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J1901-04/dspsr_fold/J1901-04_hist_fit_paper_version.pdf}
% \figsetgrpnote{Pulse stack, Posteriors, ON/OFF histogram model fit}
% \figsetgrpend


% \figsetgrpstart
% \figsetgrpnum{3.16}
% \figsetgrptitle{PSR J1904+33}
% \figsetplot{figures/all_pulsars/J1904+33/dspsr_fold/J1904+33_profile_sps_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J1904+33/dspsr_fold/J1904+33_corner_plot_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J1904+33/dspsr_fold/J1904+33_hist_fit_paper_version.pdf}
% \figsetgrpnote{Pulse stack, Posteriors, ON/OFF histogram model fit}
% \figsetgrpend


% \figsetgrpstart
% \figsetgrpnum{3.17}
% \figsetgrptitle{PSR J1928+28}
% \figsetplot{figures/all_pulsars/J1928+28/dspsr_fold/J1928+28_profile_sps_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J1928+28/dspsr_fold/J1928+28_corner_plot_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J1928+28/dspsr_fold/J1928+28_hist_fit_paper_version.pdf}
% \figsetgrpnote{Pulse stack, Posteriors, ON/OFF histogram model fit}
% \figsetgrpend


% \figsetgrpstart
% \figsetgrpnum{3.18}
% \figsetgrptitle{PSR J1941+02}
% \figsetplot{figures/all_pulsars/J1941+02/dspsr_fold/J1941+02_profile_sps_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J1941+02/dspsr_fold/J1941+02_corner_plot_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J1941+02/dspsr_fold/J1941+02_hist_fit_paper_version.pdf}
% \figsetgrpnote{Pulse stack, Posteriors, ON/OFF histogram model fit}
% \figsetgrpend


% \figsetgrpstart
% \figsetgrpnum{3.19}
% \figsetgrptitle{PSR J2000+29}
% \figsetplot{figures/all_pulsars/J2000+29/dspsr_fold/J2000+29_profile_sps_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J2000+29/dspsr_fold/J2000+29_corner_plot_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J2000+29/dspsr_fold/J2000+29_hist_fit_paper_version.pdf}
% \figsetgrpnote{Pulse stack, Posteriors, ON/OFF histogram model fit}
% \figsetgrpend


% \figsetgrpstart
% \figsetgrpnum{3.20}
% \figsetgrptitle{PSR J2040$-$21}
% \figsetplot{figures/all_pulsars/J2040-21/dspsr_fold/J2040-21_profile_sps_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J2040-21/dspsr_fold/J2040-21_corner_plot_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J2040-21/dspsr_fold/J2040-21_hist_fit_paper_version.pdf}
% \figsetgrpnote{Pulse stack, Posteriors, ON/OFF histogram model fit}
% \figsetgrpend


% \figsetgrpstart
% \figsetgrpnum{3.21}
% \figsetgrptitle{PSR J2044+28}
% \figsetplot{figures/all_pulsars/J2044+28/dspsr_fold/J2044+28_profile_sps_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J2044+28/dspsr_fold/J2044+28_corner_plot_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J2044+28/dspsr_fold/J2044+28_hist_fit_paper_version.pdf}
% \figsetgrpnote{Pulse stack, Posteriors, ON/OFF histogram model fit}
% \figsetgrpend


% \figsetgrpstart
% \figsetgrpnum{3.22}
% \figsetgrptitle{PSR J2131$-$31}
% \figsetplot{figures/all_pulsars/J2131-31/dspsr_fold/J2131-31_profile_sps_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J2131-31/dspsr_fold/J2131-31_corner_plot_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J2131-31/dspsr_fold/J2131-31_hist_fit_paper_version.pdf}
% \figsetgrpnote{Pulse stack, Posteriors, ON/OFF histogram model fit}
% \figsetgrpend


% \figsetgrpstart
% \figsetgrpnum{3.23}
% \figsetgrptitle{PSR J2310+6706}
% \figsetplot{figures/all_pulsars/J2310+6706/dspsr_fold/J2310+6706_profile_sps_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J2310+6706/dspsr_fold/J2310+6706_corner_plot_paper_version.pdf}
% \figsetplot{figures/all_pulsars/J2310+6706/dspsr_fold/J2310+6706_hist_fit_paper_version.pdf}
% \figsetgrpnote{Pulse stack, Posteriors, ON/OFF histogram model fit}
% \figsetgrpend

==> nulling_param.tex <==
\begin{deluxetable*}{clllcDccc}[h]\label{tab:nf_res}
\tablehead{\colhead{Pulsar} & \colhead{Period} & \colhead{Period derivative} & \colhead{DM} & \colhead{NF}  & \multicolumn{2}{c}{NF (Ritchings)} & \colhead{Null period} & \multicolumn{2}{c}{Lengths}\\
\colhead{} & \colhead{} & \colhead{} & \colhead{} & \colhead{} & \colhead{}  & \colhead{} & \colhead{} & \colhead{Null} & \colhead{Emission}\\
\cline{9-10}\\
\colhead{} & \colhead{(s)} & \colhead{($10^{-15}$\,s/s)} & \colhead{(pc/${\rm cm}^3$)} & \colhead{(\%)} & \multicolumn{2}{c}{(\%)} & \colhead{} & \colhead{} & \colhead{}}
\decimals
\startdata
\sidehead{GBT sample}
J0054+6946\tablenotemark{a} & 0.832911328744(4) & $-$0.7194(8) & 116.34(3) & 38.74\plmi1.1 & 36.77 & \nodata & 2 & 3 \\
J0111+6624\tablenotemark{a} & 4.3018721007(3) & $-$8.4(2) & 111.19(9) & 10.18\plmi1.66 & 17.89 & \nodata & 2 & 7 \\
J0325+6744\tablenotemark{a} & 1.36467876728(1) & $-$1.553(9) & 65.46(4) & 53.79\plmi0.79 & 55.11 & \nodata & 3 & 4 \\
J0414+31\phm{00} & 1.08051238(4) & \nodata & 64.42(7) & 27.53\plmi1.95 & 40.73 & $28.44_{-3.16}^{+12.64}$ & 2 & 4 \\
J0614+83\phm{00} & 1.03918811(9) & \nodata & 45(5) & 6.73\plmi3.12 & 52.35 & \nodata & 1-2\tablenotemark{b} & \nodata\\
J0738+6904\tablenotemark{a} & 6.8276928023(5) & $-$26.97(4) & 17.24(1) & 66.46\plmi1.46 & 64.92 & $42.67_{-7.11}^{+7.11}$ & 9 & 4 \\
J1529$-$26\phm{00} & 0.79857100(5) & \nodata & 44.7(1) & 2.52\plmi4.29 & 48.47 & \nodata & 1-2\tablenotemark{b} & \nodata \\
J1536$-$30\phm{00} & 1.90084145(9) & \nodata & 63.37(7) & 43.79\plmi2.22 & 57.46 & \nodata & 4 &  \\
J1629+33\phm{00} & 1.5247314(5) & \nodata & 34.0(7) & 83.8\plmi1.94 & 83.88 & \nodata & 12 & 1-2\tablenotemark{b}\\
J1821+4147\tablenotemark{a} & 1.261857209133(9) & $-$1.7292(9) & 40.63(5) & 0.02\plmi0.56 & 20.93 & \nodata & 1-2\tablenotemark{b} & \nodata\\
J1829+25\phm{00} & 2.8576922(1) & \nodata & 73.6(1) & 0.03\plmi0.55 & 7.81 & \nodata & 0\tablenotemark{c} & \nodata\\
J1901$-$04\phm{00} & 1.8255461(8) & \nodata & 106.2(9) & 13.94\plmi4.11 & 49.69 & $3.61_{-0.05}^{+0.05}$\tablenotemark{d} & 1\tablenotemark{b} & \nodata \\
J2040$-$21\phm{00} & 0.562564127(4) & \nodata & 23.76(1) & 25.45\plmi1.8 & 42.37 & $23.27_{-6.35}^{+4.23}$ & 2 & 5\\
J2131$-$31\phm{00} & 3.325371(5) & \nodata & 31.753 & 49.82\plmi8.63 & 54.18 & \nodata & 3 & 3\\
J2310+6706\tablenotemark{a} & 1.944788973(1) & $-$0.06(5) & 97.8(1) & 54.1\plmi2.7 & 98.99 & $3.01_{-0.04}^{+0.07}$ & 3 & 3\\
\hline
\sidehead{AO sample}
J0355+28\phm{00} & 0.36492919909(3) & \nodata & 49.38(2) & 1.64\plmi1.09 & 30.35 & \nodata & 1-2\tablenotemark{b} & \nodata\\
J0414+31\phm{00} & 1.0805124699(3) & \nodata & 65.414 & 32.99\plmi0.75 & 36.94 & $28.44_{-6.32}^{+3.16}$ & 2 & 4 \\
J1822+02\phm{00} & 1.5081132778(9) & $-$0.120(4) & 103.73(8) & 0.13\plmi0.71 & 9.26 & \nodata & 1\tablenotemark{b} & \nodata\\
J1829+25\phm{00} & 2.8576921(1) & $-$1.8(5) & 73.8(1) & 0.02\plmi0.62 & 5.54 & \nodata & 0\tablenotemark{c} & \nodata\\
J1904+33\phm{00} & 0.417032327(1) & $-$0.247(5) & 81.28(3) & 0.0\plmi0.09 & 9.44 & \nodata  & 1\tablenotemark{b} & \nodata\\
J1928+28\phm{00}  &  1.0630373062(5) & \nodata &
79.34  & 47.61\plmi2.42 &   71.87 & \nodata &    3.0 & 3.0 \\
J1941+02\phm{00} & 1.23229077(1) & $-$0.18(9) & 87.478 & 0.17\plmi1.69 & 31.12 & \nodata & 1-3\tablenotemark{b} & \nodata\\
J2000+29\phm{00} & 3.07377646(2) & $-$37.37(8) & 132.62 & 19.26\plmi1.13 & 23.4 & \nodata & 1-2\tablenotemark{b} & 3 \\
J2044+28\phm{00} & 1.61816650(1) & $-$3.99(4) & 90.169 & 15.17\plmi0.89 & 17.4 & \nodata & 1-2\tablenotemark{b} & 6\\
\enddata
\tablenotetext{a}{Adapted from \citet{Lynch2018}}
\tablenotetext{b}{We find that in extreme cases (non-nulling/highly-nulling), one of the distributions is confined to very few bins and so we quote the this range rather than fitting for it.}
\tablenotetext{c}{We find that there are no single pulses with NP$>$0.5}
\tablenotetext{d}{We observe power at integer and fractional harmonics in addition to fundamental frequency.}
\end{deluxetable*}
